Photo-z Estimation: An Example of Nonparametric Conditional Density Estimation under Selection Bias

Redshift is a key quantity for inferring cosmological model parameters. In photometric redshift estimation, cosmologists use the coarse data collected from the vast majority of galaxies to predict the redshift of individual galaxies. To properly quantify the uncertainty in the predictions, however, one needs to go beyond standard regression and instead estimate the full conditional density f(z|x) of a galaxy's redshift z given its photometric covariates x. The problem is further complicated by selection bias: usually only the rarest and brightest galaxies have known redshifts, and these galaxies have characteristics and measured covariates that do not necessarily match those of more numerous and dimmer galaxies of unknown redshift. Unfortunately, there is not much research on how to best estimate complex multivariate densities in such settings. Here we describe a general framework for properly constructing and assessing nonparametric conditional density estimators under selection bias, and for combining two or more estimators for optimal performance. We propose new improved photo-z estimators and illus- trate our methods on data from the Sloan Data Sky Survey and an application to galaxy-galaxy lensing. Although our main application is photo-z estimation, our methods are relevant to any high-dimensional regression setting with complicated asymmetric and multimodal distributions in the response variable.

==> algorithm.tex <==

\red{I'm still working on the algorithm}

\begin{algorithm}
	\caption{ \small Redshift Estimation Under Selection Bias}\label{algorithmCondReg}
	\algorithmicrequire \ {\small Training labeled data
		$(\x_1^L,z_1^L),\ldots,(\x_{n_L}^L,z_{n_L}^L)$; \\
		Validation labeled data
		$(\tilde{\x}_1^L,\tilde{z}_1^L),\ldots,
		(\tilde{\x}_{\tilde{n_L}}^L,\tilde{z}_{\tilde{n_L}}^L)$; \\ Training unlabeled data
		$\x_1^U,\ldots,\x_{n_U}^U$; \\
		Validation unlabeled data
		$\tilde{\x}_1^U,\ldots,
		\tilde{\x}_{\tilde{n_U}}^U$
		 \\
		validation data; grid over $\epsilon$, $I$ and $J$. } %Due to the orthogonality of the spectral basis,
	%\Comment{$\epsilon$'s are the tuning parameters associated with the kernel}
	
	\algorithmicensure \ {\small Estimator $\widehat{f}(z|\vec{x})$}
	\begin{algorithmic}[1]
		\State Find the best estimator of the importance weights $\beta$ by minimizing the estimated loss of Eq.~\ref{eq-lossBetaEst}
		\State Variable Selection
		\State Find the best estimator of the conditional density $f(z|\x)$ by minimizing the estimated loss of \ref{eq-lossCDEEstimate}
%		\ForAll{$\epsilon$}
%		\State calculate the eigenvectors $\widetilde{\psi}=\widetilde{\psi}_{\epsilon}$ of the Gram matrix \Comment{Eq.~(\ref{gramMatrix})}
%		\State estimate the eigenbasis $\widehat{\Psi}_{i,j}$ \Comment{Eq.~(\ref{PsiEstimate})}
%		\State estimate the coefficients $\widehat{\beta}_{i,j}$ \Comment{Eq.~(\ref{beta})}
%		\ForAll{$I,J$}
%		\State calculate the estimated loss $\widehat{L}(\widehat{f}_{\epsilon,I,J},f)$ \Comment{Eq.~(\ref{lossEmpirical})} 
%		\EndFor
%		\EndFor
%		\State Define $\widehat{f}=\arg \min_{\widehat{f}_{\epsilon,I,J}(z|\vec{x})} \widehat{L}(\widehat{f}_{\epsilon,I,J},f)$
%		%     \State Calculate $\widetilde{f}$, the renormalization of $\widehat{f}$ \Comment{Sec.~\ref{normalization}}
%		\State \textbf{return} $\widehat{f}(z|\vec{x})$
%		
	\end{algorithmic}
\end{algorithm}
